Task-oriented Prompt Enhancement via Script Generation

Large Language Models (LLMs) have demonstrated remarkable abilities across various tasks, leveraging advanced reasoning. Yet, they struggle with task-oriented prompts due to a lack of specific prior knowledge of the task answers. The current state-of-the-art approach, PAL, utilizes code generation to address this issue. However, PAL depends on manually crafted prompt templates and examples while still producing inaccurate results. In this work, we present TITAN-a novel strategy designed to enhance LLMs' performance on task-oriented prompts. TITAN achieves this by generating scripts using a universal approach and zero-shot learning. Unlike existing methods, TITAN eliminates the need for detailed task-specific instructions and extensive manual efforts. TITAN enhances LLMs' performance on various tasks by utilizing their analytical and code-generation capabilities in a streamlined process. TITAN employs two key techniques: (1) step-back prompting to extract the task's input specifications and (2) chain-of-thought prompting to identify required procedural steps. This information is used to improve the LLMs' code-generation process. TITAN further refines the generated script through post-processing and the script is executed to retrieve the final answer. Our comprehensive evaluation demonstrates TITAN's effectiveness in a diverse set of tasks. On average, TITAN outperforms the state-of-the-art zero-shot approach by 7.6% and 3.9% when paired with GPT-3.5 and GPT-4. Overall, without human annotation, TITAN achieves state-of-the-art performance in 8 out of 11 cases while only marginally losing to few-shot approaches (which needed human intervention) on three occasions by small margins. This work represents a significant advancement in addressing task-oriented prompts, offering a novel solution for effectively utilizing LLMs in everyday life tasks.

==> tabs/Math_Result.tex <==

\begin{table*}[t]
    \centering
    \caption{
    Comparison of \tool accuracy (\%) to other code generation approaches,
    %of correctly solved 
    %mathematical, symbolic, and task-oriented 
    %problems, 
    evaluated across eleven benchmarks using two GPT models.
    %versions with greedy decoding. 
    %PAL ZS represents PAL with zero-shot prompting; PAL FS represents PAL with few-shot prompting; MS represents Model Selection~\cite{zhao2023automatic}; XoT represents X-of-Thoughts~\cite{liu2023plan}. 
    The 
    %asterisk 
    $^*$ symbol 
    %above the approach 
    indicates the accuracy is from 
    %that we have adopted the value from 
    %the 
    original papers.
    %, as the code was not accessible. 
    %The $\uparrow$, $\downarrow$ and - indicate improvement, how our method fares in comparison to the top results achieved by other approaches. 
    The best accuracy scores for each dataset and model are 
    %emphasized in 
    bold.
    }
    \label{tab:math_result}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l r@{ }c r@{ }c r@{ }c r@{ }c r@{}c@{}c r@{ }c r@{ }c r@{ }c r@{}c@{}c}
        \toprule
         LLM &  \multicolumn{11}{c}{GPT-3.5} &  \multicolumn{9}{c}{GPT-4}\\
         
         \cmidrule(lr){1-1} \cmidrule(lr){2-12} \cmidrule(lr){13-21}
         
         Approach 
         &\multicolumn{2}{c}{PAL ZS} 
         &\multicolumn{2}{c}{PAL}
         &\multicolumn{2}{c}{MS$^{*}$}
         &\multicolumn{2}{c}{XoT$^{*}$}
         &\multicolumn{3}{c}{\textbf{\tool}}
         &\multicolumn{2}{c}{PAL ZS}
         &\multicolumn{2}{c}{PAL}
         &\multicolumn{2}{c}{MS$^{*}$}
         &\multicolumn{3}{c}{\textbf{\tool}}\\
         
         Zero-shot
         &\multicolumn{2}{c}{\ding{51}}
         &\multicolumn{2}{c}{\ding{55}}
         &\multicolumn{2}{c}{\ding{55}}
         &\multicolumn{2}{c}{\ding{55}}
         &\multicolumn{3}{c}{\ding{51}}
         &\multicolumn{2}{c}{\ding{51}}
         &\multicolumn{2}{c}{\ding{55}}
         &\multicolumn{2}{c}{\ding{55}}
         &\multicolumn{3}{c}{\ding{51}}\\

         \cmidrule(lr){1-1}
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
         \cmidrule(lr){13-14} \cmidrule(lr){15-16} \cmidrule(lr){17-18} \cmidrule(lr){19-21}

         Metric
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$Z\Delta$} & \multicolumn{1}{c}{$A\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$T\Delta$}
         & \multicolumn{1}{c}{$Acc$} & \multicolumn{1}{c}{$Z\Delta$} & \multicolumn{1}{c}{$A\Delta$}\\
         
         \cmidrule(lr){1-1} \cmidrule(lr){2-12} \cmidrule(lr){13-21}
         
         GSM8K &  76.6&\textcolor{OrangeRed}{$\downarrow$7.6} & 81.0&\textcolor{OrangeRed}{$\downarrow$3.2} & 82.6 &\textcolor{OrangeRed}{$\downarrow$1.6} & 83.3&\textcolor{OrangeRed}{$\downarrow$0.9}
         &\textbf{84.2}&\textcolor{ForestGreen}{$\uparrow$7.6}&\textcolor{ForestGreen}{$\uparrow$0.9}
         & 93.6&\textcolor{OrangeRed}{$\downarrow$1.7}& 94.8&\textcolor{OrangeRed}{$\downarrow$0.5}& \textbf{95.6}&\textcolor{ForestGreen}{$\uparrow$0.3}
         & 95.3&\textcolor{ForestGreen}{$\uparrow$1.7}&\textcolor{OrangeRed}{$\downarrow$0.3}\\
         
         GSMHard&  61.8& \textcolor{OrangeRed}{$\downarrow$7.8}&  64.1& \textcolor{OrangeRed}{$\downarrow$5.5}&  -& &  63.4& \textcolor{OrangeRed}{$\downarrow$6.2}
         &\textbf{69.6}&\textcolor{ForestGreen}{$\uparrow$7.8}&\textcolor{ForestGreen}{$\uparrow$5.5}
         &  74.1& \textcolor{OrangeRed}{$\downarrow$4.1}&  70.9& \textcolor{OrangeRed}{$\downarrow$7.3}&  -& 
         &\textbf{78.2}&\textcolor{ForestGreen}{$\uparrow$4.1}&\textcolor{ForestGreen}{$\uparrow$4.1}\\
         
         ASDIV&  85.3& \textcolor{OrangeRed}{$\downarrow$6.1}&  86.4& \textcolor{OrangeRed}{$\downarrow$5.0}&  89.4& \textcolor{OrangeRed}{$\downarrow$2.0}&  -&
         &\textbf{91.4}&\textcolor{ForestGreen}{$\uparrow$6.1}&\textcolor{ForestGreen}{$\uparrow$2.0}
         &  92.7& \textcolor{OrangeRed}{$\downarrow$4.5}&  92.1& \textcolor{OrangeRed}{$\downarrow$5.1}&  93.5& \textcolor{OrangeRed}{$\downarrow$3.7}
         &\textbf{97.2}&\textcolor{ForestGreen}{$\uparrow$4.5}&\textcolor{ForestGreen}{$\uparrow$3.7}\\
         
         SVAMP&  82.8& \textcolor{OrangeRed}{$\downarrow$1.5}&  \textbf{84.6}& \textcolor{ForestGreen}{$\uparrow$0.3}&  84.3&          \textcolor{Gray}{-0.0}&  83.6& \textcolor{OrangeRed}{$\downarrow$0.7}
         &84.3&\textcolor{ForestGreen}{$\uparrow$1.5}&\textcolor{OrangeRed}{$\downarrow$0.3}
         &  94.0& \textcolor{OrangeRed}{$\downarrow$0.8}&  94.6& \textcolor{OrangeRed}{$\downarrow$0.2}&  93.7& \textcolor{OrangeRed}{$\downarrow$1.1}
         &\textbf{94.8}&\textcolor{ForestGreen}{$\uparrow$0.8}&\textcolor{ForestGreen}{$\uparrow$0.2}\\
         
         AddSub&  \textbf{93.1}& \textcolor{ForestGreen}{$\uparrow$3.3}&  92.7& \textcolor{ForestGreen}{$\uparrow$2.9}&  90.6&          \textcolor{ForestGreen}{$\uparrow$0.8}&  90.5& \textcolor{ForestGreen}{$\uparrow$0.7}
         &89.8&\textcolor{OrangeRed}{$\downarrow$3.3}&\textcolor{OrangeRed}{$\downarrow$3.3}
         &  95.7& \textcolor{OrangeRed}{$\downarrow$2.0}&  97.2& \textcolor{OrangeRed}{$\downarrow$0.5}&  95.7& \textcolor{OrangeRed}{$\downarrow$2.0}
         &\textbf{97.7}&\textcolor{ForestGreen}{$\uparrow$2.0}&\textcolor{ForestGreen}{$\uparrow$0.5}\\
         
         Multiarith&  97.3&\textcolor{ForestGreen}{$\uparrow$0.5}&  \textbf{98.7}& \textcolor{ForestGreen}{$\uparrow$1.9}&  98.7&          \textcolor{ForestGreen}{$\uparrow$1.9}& 97.3&\textcolor{ForestGreen}{$\uparrow$0.5}
         &96.8&\textcolor{OrangeRed}{$\downarrow$0.5}&\textcolor{OrangeRed}{$\downarrow$1.9}
         &96.8& \textcolor{OrangeRed}{$\downarrow$1.9}&  98.8& \textcolor{ForestGreen}{$\uparrow$0.1}&  \textbf{99.0}& \textcolor{ForestGreen}{$\uparrow$0.3}
         &98.7&\textcolor{ForestGreen}{$\uparrow$1.9}&\textcolor{OrangeRed}{$\downarrow$0.3}\\
         
         Penguin&  59.1&\textcolor{OrangeRed}{$\downarrow$35.2}&\textbf{96.6}&\textcolor{ForestGreen}{$\uparrow$2.3}&  -&   &  -&         
         &94.3&\textcolor{ForestGreen}{$\uparrow$35.2}&\textcolor{OrangeRed}{$\downarrow$2.3}
         &  87.2& \textcolor{OrangeRed}{$\downarrow$10.3}&  96.6&          \textcolor{OrangeRed}{$\downarrow$0.9}&  -&         
         &\textbf{97.5}&\textcolor{ForestGreen}{$\uparrow$10.3}&\textcolor{ForestGreen}{$\uparrow$0.9}\\

        \cmidrule(lr){1-1} \cmidrule(lr){2-12} \cmidrule(lr){13-21}
         
         Finding& 93.8& \textcolor{OrangeRed}{$\downarrow$4.6}& 97.7& \textcolor{OrangeRed}{$\downarrow$0.7}& -&& -&
         &\textbf{98.4}&\textcolor{ForestGreen}{$\uparrow$4.6}&\textcolor{ForestGreen}{$\uparrow$0.7}
         & 95.5& \textcolor{OrangeRed}{$\downarrow$4.3}& \textbf{99.8}&         \textcolor{Gray}{-0.0}& -&
         &\textbf{99.8}&\textcolor{ForestGreen}{$\uparrow$4.3}&\textcolor{Gray}{-0.0}\\
         
         Counting& \textbf{89.1}& \textcolor{ForestGreen}{$\uparrow$1.3}& 84.6& \textcolor{OrangeRed}{$\downarrow$3.2}& -&& -&
         &87.8&\textcolor{OrangeRed}{$\downarrow$1.3}&\textcolor{OrangeRed}{$\downarrow$1.3}
         & 87.5& \textcolor{OrangeRed}{$\downarrow$2.3}& 88.5& \textcolor{OrangeRed}{$\downarrow$1.3}& -&
         &\textbf{89.8}&\textcolor{ForestGreen}{$\uparrow$2.3}&\textcolor{ForestGreen}{$\uparrow$1.3}\\
         
         True/False& 59.2& \textcolor{OrangeRed}{$\downarrow$17.5}& 76.0& \textcolor{OrangeRed}{$\downarrow$0.7}& -&& -&
         &\textbf{76.7}&\textcolor{ForestGreen}{$\uparrow$17.5}&\textcolor{ForestGreen}{$\uparrow$0.7}
         & 84.4& \textcolor{OrangeRed}{$\downarrow$9.4}& \textbf{95.6}& \textcolor{ForestGreen}{$\uparrow$1.8}& -&
         &93.8&\textcolor{ForestGreen}{$\uparrow$9.4}&\textcolor{OrangeRed}{$\downarrow$1.8}\\
         
         Generative& 84.9& \textcolor{OrangeRed}{$\downarrow$9.2}& 87.7& \textcolor{OrangeRed}{$\downarrow$6.4}& -&& -&
         &\textbf{94.1}&\textcolor{ForestGreen}{$\uparrow$9.2}&\textcolor{ForestGreen}{$\uparrow$6.4}
         & 98.7& \textcolor{OrangeRed}{$\downarrow$1.2}& 99.4& \textcolor{OrangeRed}{$\downarrow$0.5}& -&
         &\textbf{99.9}&\textcolor{ForestGreen}{$\uparrow$1.2}&\textcolor{ForestGreen}{$\uparrow$0.5}\\
         
        \cmidrule(lr){1-1} \cmidrule(lr){2-12} \cmidrule(lr){13-21}
        
        Average & 80.3&\textcolor{OrangeRed}{$\downarrow$7.6} 
        & 86.4&\textcolor{OrangeRed}{$\downarrow$1.5}
        & -& %\textcolor{OrangeRed}{-0.1}
        & -& %\textcolor{OrangeRed}{-0.9}
        & \textbf{87.9}&\textcolor{ForestGreen}{$\uparrow$7.6}&\textcolor{ForestGreen}{$\uparrow$1.5} 
        & 90.9&\textcolor{OrangeRed}{$\downarrow$3.9} 
        & 93.5&\textcolor{OrangeRed}{$\downarrow$1.3}& -&%\textcolor{OrangeRed}{-0.9}
        &\textbf{94.8}&\textcolor{ForestGreen}{$\uparrow$3.9}&\textcolor{ForestGreen}{$\uparrow$1.3}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-5pt}
\end{table*}
